Topology-Aware Network Pruning using Multi-stage Graph Embedding and Reinforcement Learning

Model compression is an essential technique for deploying deep neural networks (DNNs) on power and memory-constrained resources. However, existing model-compression methods often rely on human expertise and focus on parameters' local importance, ignoring the rich topology information within DNNs. In this paper, we propose a novel multi-stage graph embedding technique based on graph neural networks (GNNs) to identify DNN topologies and use reinforcement learning (RL) to find a suitable compression policy. We performed resource-constrained (i.e., FLOPs) channel pruning and compared our approach with state-of-the-art model compression methods. We evaluated our method on various models from typical to mobile-friendly networks, such as ResNet family, VGG-16, MobileNet-v1/v2, and ShuffleNet. Results show that our method can achieve higher compression ratios with a minimal fine-tuning cost yet yields outstanding and competitive performance.

==> contents/06_impact.tex <==
\section*{Broader impacts}
Neural network compression and particularly network pruning can greatly reduce the runtime and memory footprint of deep networks. Given the potential to consume less energy, such methods can also alleviate the negative environmental impact of wide-spreading AI applications. We believe that our proposed method can facilitate neural network deployment and positively impact the required energy for running deep networks.

==> contents/a01_algorithm_environment.tex <==
\begin{algorithm}[H]
    \caption{Graph environment algorithm in one search episodes }
    \label{alg}
\begin{algorithmic}\small

\STATE {\bfseries Input:} The DNN $M$ and the desired model size $d$.
\STATE {\bfseries Output:} The pruned DNN $M$.

\WHILE{$Size(M) > d$}
    
    \STATE $s = Graph\_Generator(M)$
    \STATE $a = PPO.Actor\_Critic(s)$
    \STATE $PPO.Memory(s,a)$
    \STATE $M \leftarrow Pruner(a,M)$
\ENDWHILE
\STATE $R_{err} = -Error(M)$
\STATE $PPO.update(R_{err})$

\STATE {\bfseries Return} $M$

\end{algorithmic}
\end{algorithm}


==> contents/f03_figure3.tex <==
\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.9\columnwidth]{figures/figure3.png}}
\caption{We convert the 3x3 convolution with three input channels and four output channels to a 2-levels hierarchical graph. The level 1 graph $G^1$ denotes the operation of a 3 input channel 3x3 convolutional filter. The level 2 graph $G^2$ denotes the operations 4 of those filters.}
\label{fig:3}
\end{center}
\vskip -0.2in
\end{figure}

==> contents/f06_figure6.tex <==
\begin{figure}[t]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/point-depth.png}}
\caption{An example for pruning depth-wise filters on MobileNet-v1 blocks.}
\label{fig:6}
\end{center}
\vskip -0.2in
\end{figure}

% A MobileNet-v1 block contains a depth-wise convolution layer and a point-wise convolution layer. As shown in the figure, we prune a depth-wise filter (painted gray) that causes its corresponding channel's information loss (painted green).

==> contents/t01_overparameterized_DNN_CIFAR.tex <==
\begin{table}[t]
\caption{Top-1 Classification accuracy for pruned over-parameterized DNNs on CIFAR-10. The original ResNet-110/56/44/32/20 are pre-trained on CIFAR-10 with Top-1 test accuracy of 93.68\%, 93.39\%, 93.10\%, 92.63\%, and 91.73\%, respectively.}
\label{table_op_cifar}
\vspace{-10pt}
\begin{center}
\begin{small}
\begin{sc}

\begin{tabular}{lccccccr}
\toprule
model  &dataset & method &flops $\downarrow$ \% & Orig. $Acc.\%$ &Pruned $Acc.\%$ & $\Delta Acc.$ \\
\midrule
\multirow{3}{*}{ResNet110} & \multirow{3}{*}{CIFAR-10}   &agmc   & $50\%$  & 93.14 & $ 93.08$     & $-0.6 $\\
                             & &rs     & $50\%$ & 93.14 &  $87.26 $    & $ -6.42$ \\
                             & &\textbf{gnn-rl} & $52\%$  & 93.14& $\textbf{94.31}$ & $\textbf{+0.63}$ \\
\midrule
\multirow{5}{*}{ResNet56}    &\multirow{5}{*}{CIFAR-10} &uniform& $50\%$  & 93.39 & $87.5$ & $-5.89$ \\
                             & &deep   & $50\%$  & 93.39& $88.40$ & $-4.99$ \\
                             & &amc    & $50\%$  & 93.39& $90.20$ & $-3.19$ \\
                             & &agmc   & $50\%$  &93.39 & $92.00$ & $-1.39$\\
                             & &\textbf{gnn-rl} & $54\%$  & 93.39& $\textbf{93.49}$ & $\textbf{+0.1}$ \\
\midrule
\multirow{3}{*}{ResNet44}    &\multirow{3}{*}{CIFAR-10} &agmc   & $50\%$  &93.10 &  $92.28$ & $-0.82 $ \\
                             & &rs     & $50\%$  & 93.10&  $ 88.14$ & $-4.96 $ \\
                             & &\textbf{gnn-rl} & $51\%$  &93.10 &  $\textbf{93.23}$ & $\textbf{+0.13}$ \\
\midrule
\multirow{3}{*}{ResNet32}    & \multirow{3}{*}{CIFAR-10}&agmc   & $50\%$  &92.63 &  $90.96$ & $-1.67$ \\
                             & &rs     & $50\%$  & 92.63&  $ 89.57$ & $-3.06$ \\
                             & &\textbf{gnn-rl} & $51$\%  &92.63  & $\textbf{92.58}$ & $-0.05$ \\
\midrule
\multirow{5}{*}{ResNet20}    &\multirow{5}{*}{CIFAR-10} &deep   & $50\%$  &91.73 &  $79.60$ & $-12.13$ \\
                             & &shallow& $50\%$  &91.73 &  $83.20$ & $-8.53$ \\
                             & &uniform& $50\%$  &91.73 &  $84.00$ & $-7.73$ \\
                             & &amc    & $50\%$  &91.73 &  $86.40$ & $-5.33$ \\
                             & &agmc   & $50\%$  &91.73 &  $88.42$ & $-3.31$ \\
                             & &\textbf{gnn-rl} & $51\%$  &91.73 &  $\textbf{91.31}$ & $-0.42$ \\

\midrule
\multirow{3}{*}{ShuffleNet-v1} &\multirow{3}{*}{CIFAR-100} &agmc   &  $40\%$ &69.94 & $65.26 $     & $ -3.38$\\
                                & &rs     &  $40\%$ & 69.94&  $63.70 $    & $ -4.94$ \\
                                & &\textbf{gnn-rl} & $42\% $ & 69.94& $ \textbf{67.10} $ & $ -2.84 $ \\
\midrule
\multirow{3}{*}{ShuffleNet-v2} 
                            &\multirow{3}{*}{CIFAR-100} &agmc    & $40\%$  & 68.85& $ 66.28$ & $-2.57 $ \\
                            &  &rs   &  $40\%$& 68.85 & $ 65.74$ & $ -3.11$\\
                            &  &\textbf{gnn-rl} & $46\% $  & 68.85& $\textbf{66.64}$ & $-2.21$ \\
                            
\bottomrule
\end{tabular}
\end{sc}

\end{small}

\end{center}
\vspace{-15pt}
\end{table}


==> contents/t02_overparameterized_DNN_imgnet.tex <==
\begin{table}[t]
\caption{Top-1 Classification accuracy for pruned over-parameterized DNNs on ImageNet. The original VGG-16 is pre-trained on ImageNet with Top-1 test accuracy of 70.5\%. }
\label{table_op_imagenet}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccccr}
\toprule
model  & method &flops $\downarrow$ \% & Orig. $Acc.\%$ &Pruned $Acc.\%$ & $\Delta Acc.$ \\
\midrule
\multirow{4}{*}{VGG-16}        &fp & 80    &70.50& $55.90$ & $-14.6$ \\
                               &rnp & 80    &70.50& $66.92$ & $-3.58$ \\
                               &spp & 80    &70.50& $68.20$ & $-2.30$ \\
                             &amc & 80    &70.50& $69.10$ & $-1.40$ \\
                               &\textbf{gnn-rl} & 80    &70.50& $ \textbf{70.99}$ & $+0.49$ \\
\midrule
\multirow{4}{*}{ResNet-18}        & FPGM &  $42$   &70.28& 68.41  & -1.87  \\
                               &  SFP&    $42$  &70.28& 67.10  & -3.18 \\
                                &  PFP-B    & $43$  &69.74& 65.65 & -4.09 \\
                            &DMCP & 42    &70.10& $ 69.20$ & $-0.90$ \\
                               &\textbf{gnn-rl} &   $25$   &69.76& 68.66  & -1.10   \\
                                &\textbf{gnn-rl} &   $51$   &69.76& 67.62  &-2.14   \\
\midrule
\multirow{5}{*}{ResNet-50}        & AutoPruner &   48  &76.15& 74.76  & -1.39  \\
                               & Meta-Pruning&   50   &76.60& 73.40  &  -3.20  \\
                               & AutoSlim &    50  &76.10  &   74.00 & -2.10\\
                               &LeGR        &  42   & 76.10 & 75.70&-0.40 \\
                               &EagleEye        &  50   & - & 74.20& - \\
                               &DMCP        &  50   & 76.60 & 74.40& -2.20 \\
                               &{gnn-rl} &  \textbf{53} &76.10& 74.28  & -1.82 \\

\midrule
\multirow{7}{*}{MobileNet-v1}     &Uniform~\cite{Andrew2017MobileNetv1}   &  $25$  & 70.60&  $68.40 $ & $ -2.20 $ \\
                              &NetAdapt   &  $34$   &70.60 &  $69.10 $ & $  -1.50$ \\
                              &AMC~\cite{he2018amc}     &  $34$   &70.90 &  $ 70.50$ & $ -0.40$ \\
                              &Meta-Pruning~\cite{}     &  $35$  &70.60 &  $ 70.60$ & $ 0$ \\
                              &EagleEye &  $25$  &- &  $70.90 $ & - \\
                              &\textbf{gnn-rl} & $30$  &70.90 &$70.70$ & $-0.20 $ \\
                              &AMC~\cite{he2018amc}     &  $60$  &70.90 &  $ 68.90$ & $ -2.00$ \\
                              &\textbf{gnn-rl} & \textbf{ 60}  &70.90 &  $\textbf{ 69.50}$ & $ -1.40$ \\
\midrule
\multirow{3}{*}{MobileNet-v2}     &AMC   & $27$  &$71.80$ &  $70.80 $ & $ -1.00$ \\
                              &Meta-Pruning     &  $27$ & $74.70$ &  $71.20 $ & $ -3.50$ \\
                              &LeGR     &  $30$ & $71.80$ &  $71.40 $ & $ -0.40$ \\
                              &DMCP     &  $25$ & $73.90$ &  $72.40 $ & $ -1.50$ \\
                              &{gnn-rl} &  $ 42  $  & $71.80$ & $68.84 $ & $ -2.96$ \\
                              &{gnn-rl} &  $ 26  $  & $71.80$ & $69.89 $ & $ -1.91$ \\



                            
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> contents/t02_table2.tex <==
\begin{table}[t]
\caption{Top-1 Classification accuracies for pruned mobile-friendly DNNs. The original MobileNet-v1/v2 and ShuffleNet-v1/v2 are pre-trained on CIFAR-100 with Top-1 test accuracy of 64.88\%, 65.74\%, 68.64\%, and 68.85\%, respectively. The column FLOPs is the preserved FLOPs ratio compared with the original model.}
\label{table_2}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccr}
\toprule
model & dataset & method &flops $\downarrow$& $Acc.\%$ & $\Delta Acc.$ \\
\midrule
\multirow{3}{*}{ShuffleNet-v1} &CIFAR-100 &agmc   &  $60\%$  & $65.26 $     & $ -3.38$\\
                                &CIFAR-100 &rs     &  $60\%$  &  $63.7 $    & $ -4.94$ \\
                                &CIFAR-100 &\textbf{gnn-rl} & $58\% $  & $ \textbf{67.1} $ & $ -2.84 $ \\
\midrule
\multirow{3}{*}{ShuffleNet-v2} 
                            &CIFAR-100 &agmc    & $60\%$   & $ 66.28$ & $-2.57 $ \\
                            &CIFAR-100 &rs   &  $60\%$  & $ 65.74$ & $ -3.11$\\
                            &CIFAR-100 &\textbf{gnn-rl} & $54\% $  & $\textbf{66.64}$ & $-2.21$ \\
\midrule
\multirow{7}{*}{MobileNet-v1}   &ImageNet &Uniform~\cite{Andrew2017MobileNetv1}   &  $25\%$   &  $68.40 $ & $  $ \\
                            &ImageNet &NetAdapt   &  $34\%$   &  $69.10 $ & $  $ \\
                            &ImageNet &AMC~\cite{he2018amc}     &  $34\%$   &  $ 70.5$ & $ $ \\
                            &ImageNet &Meta-Pruning~\cite{}     &  $35\%$   &  $ 70.6$ & $ $ \\
                            &ImageNet &EagleEye &  $25\%$   &  $70.9 $ & $ $ \\
                            &ImageNet &\textbf{gnn-rl} & $30\%$   &$70.70$ & $ $ \\
                            &ImageNet &AMC~\cite{he2018amc}     &  $60\%$   &  $ 68.9$ & $ $ \\
                            &ImageNet &\textbf{gnn-rl} & \textbf{ 60\%}  &  $\textbf{ 69.5}$ & $ $ \\
\midrule
\multirow{3}{*}{MobileNet-v2}   &ImageNet &AMC   & $27\%$   &  $70.8 $ & $ -1.0$ \\
                            &ImageNet &Meta-Pruning     &  $27\%$   &  $71.2 $ & $ -0.8$ \\
                            &ImageNet &LeGR     &  $30\%$   &  $71.4 $ & $ -0.4$ \\
                            &ImageNet &DMCP     &  $25\%$   &  $72.4 $ & $ -1.5$ \\
                            &ImageNet &\textbf{gnn-rl} &  $ 26\%  $    & $69.83 $ & $ $ \\




                            
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> contents/t04_RL.tex <==
\begin{table}[t]
\caption{RL-based methods}
\label{table_rl}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lccccr}
\toprule
Method & Policy & \# Tunable-Parameter &States space & Action space \\
\midrule
AMC & DDPG~\cite{lillicrap2016ddpg} &7 & Handcrafts & $[0,1)^N$ \\
GNN-RL & DDPG~\cite{lillicrap2016ddpg} &7 & Graph & $[0,1)^N$ \\

GNN-RL& PPO~\cite{schulman2017ppo} & 4& Graph & $[0,1)^N$ \\

                            
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.1in
\end{table}


==> contents/table_cifar.tex <==

% \begin{table}[H]

% \resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{0.91}
\begin{tabular}{llcll}
\toprule
Model    & Method                                                                                 & FLOPs $\downarrow$                                                                          & Top-1                                                                             & $\Delta$Top-1                                                                                 \\ \midrule
Res110   & \begin{tabular}[c]{@{}l@{}}AGMC\\ RS\\ PFEC\\SFP\\FPGM\\\textbf{GNN-RL}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}50\%\\ 50\%\\39\% \\41\% \\52\%\\ 52\%\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}93.08\\ 87.26\\ 93.30\\93.38\\93.74\\\textbf{94.31}\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}-0.60\\ -6.42\\-0.20\\-0.30\\+0.16\\ \textbf{+0.63}\end{tabular}                           \\ \midrule
Res56    & \begin{tabular}[c]{@{}l@{}}Uniform\\ AMC\\ FPGM\\ AGMC\\ EagleEye \\ \textbf{GNN-RL}\end{tabular}           
& \begin{tabular}[c]{@{}l@{}}50\%\\ 50\%\\59\%\\ 50\%\\ 50\%\\ \textbf{54\%}\end{tabular}        
& \begin{tabular}[c]{@{}l@{}}87.5\\  90.20\\93.26\\ 92.00\\ 94.66\\ \textbf{93.49}\end{tabular}       
& \begin{tabular}[c]{@{}l@{}}-5.89\\ -3.19\\-0.02\\ -1.39\\ +1.4\\ \textbf{+0.1}\end{tabular}           \\ \midrule
% Res44    & \begin{tabular}[c]{@{}l@{}}AGMC\\ RS\\ GNN-RL\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}50\%\\ 50\%\\ \textbf{51\%}\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}92.28\\ 88.14\\ \textbf{93.23}\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}-0.82\\ -4.96\\ \textbf{+0.13}\end{tabular}                          \\ \midrule
Res32    & \begin{tabular}[c]{@{}l@{}}AGMC\\ RS\\ SFP\\FPGM\\\textbf{GNN-RL}\end{tabular}                             
& \begin{tabular}[c]{@{}l@{}}50\%\\ 50\%\\42\%\\ 50\%\\ \textbf{51}\%\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}90.96\\ 89.57\\92.08\\91.93 \\\textbf{92.58}\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}-1.67\\ -3.06\\-0.55\\-0.70\\ \textbf{-0.05}\end{tabular}                          \\ \midrule
Res20    & \begin{tabular}[c]{@{}l@{}}Uniform\\ AMC\\ AGMC\\SFP\\FPGM\\DSA\\ \textbf{GNN-RL}\end{tabular} 
& \begin{tabular}[c]{@{}l@{}} 50\%\\ 50\%\\ 50\%\\42\%\\42\%\\50\%\\ \textbf{51\%}\end{tabular} 
& \begin{tabular}[c]{@{}l@{}} 84.00\\ 86.4\\ 88.42\\90.83\\91.09\\ 91.38\\91.31\end{tabular} & \begin{tabular}[c]{@{}l@{}} -7.73\\ -5.33\\ -3.31\\-1.37\\-1.11\\-0.79\\ \textbf{-0.42}\end{tabular} \\ \midrule
Shuff-v1 & \begin{tabular}[c]{@{}l@{}}AGMC\\ RS\\ \textbf{GNN-RL}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}40\%\\ 40\%\\ \textbf{42\%}\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}65.26\\ 63.70\\ \textbf{67.10}\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}-3.38\\ -4.94\\ -2.84\end{tabular}                          \\ \midrule
Shuff-v2 & \begin{tabular}[c]{@{}l@{}}AGMC\\ RS\\ \textbf{GNN-RL}\end{tabular}                             & \begin{tabular}[c]{@{}l@{}}40\%\\ 40\%\\ \textbf{46\%}\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}66.28\\ 65.74\\ \textbf{66.64}\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}-2.57\\ -3.11\\ -2.21\end{tabular}                        \\  
\bottomrule
\end{tabular}%
% \captionof{table}{test}
% \label{tab:res-cifar}
% }
% \end{table}

==> contents/table_imagenet.tex <==
% \begin{table}[H]
% \caption{test}
% \label{tab:res-imagenet}
% \resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.107}
\begin{tabular}{llcll}
\toprule
Model  & Method                                                                                                             & FLOPs $\downarrow$                                                                        & Top-1                                                                                                 & $\Delta$Top-1                                                                                        \\ \midrule
VGG-16 & \begin{tabular}[c]{@{}l@{}}FP\\ RNP\\ SPP\\ AMC\\AutoPruner\\ \textbf{GNN-RL}\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}80\%\\ 80\%\\ 80\%\\ 80\%\\ 74\% \\ 80\%\end{tabular}                & \begin{tabular}[c]{@{}l@{}}55.90\\ 66.92\\ 68.20\\ 69.10\\69.20 \\ \textbf{70.99}\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}-14.6\\ -3.58\\ -2.30\\ -1.40\\-2.39\\ \textbf{+0.49}\end{tabular}                 \\ \midrule
Res18  & \begin{tabular}[c]{@{}l@{}}FPGM\\ SFP\\ PFP-B\\ \textbf{GNN-RL}\end{tabular}               & \begin{tabular}[c]{@{}l@{}}42\%\\ 42\%\\ 43\%\\ \textbf{51\%}\end{tabular}           & \begin{tabular}[c]{@{}l@{}}68.41\\ 67.10\\ 65.65\\  \textbf{68.66}\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}-1.87\\ -3.18\\ -4.09\\ \textbf{-1.10}\end{tabular}         \\ \midrule
Res50  & \begin{tabular}[c]{@{}l@{}}AutoPruner\\ Meta-Pruning\\ AutoSlim\\  EagleEye\\ \textbf{GNN-RL}\end{tabular}     
& \begin{tabular}[c]{@{}l@{}}44\%\\ 50\%\\ 50\%\\  50\%\\  \textbf{53\%}\end{tabular}      
& \begin{tabular}[c]{@{}l@{}}73.84\\ 73.40\\ 74.00\\  74.20\\ \textbf{74.28}\end{tabular}
& \begin{tabular}[c]{@{}l@{}}-2.31\\ -3.20\\   N/A\\ N/A\\ \textbf{-1.82}\end{tabular}     \\ \midrule
MB-v1  & \begin{tabular}[c]{@{}l@{}}Uniform\\ NetAdapt\\ AMC\\ Meta-Pruning\\ EagleEye\\ GNN-RL\\ AMC\\ \textbf{GNN-RL}\end{tabular} & \begin{tabular}[c]{@{}l@{}}25\%\\ 34\%\\ 34\%\\ 35\%\\ 25\%\\ 30\%\\ 60\%\\ 60\%\end{tabular} & \begin{tabular}[c]{@{}l@{}}68.40\\ 69.10\\ 70.50\\ 70.60\\ 70.90\\ 70.70\\ 68.90\\ \textbf{69.50}\end{tabular} & \begin{tabular}[c]{@{}l@{}}-2.20\\ -1.50\\ -0.40\\ 0\\ N/A\\ -0.20\\ -2.00\\ \textbf{-1.40}\end{tabular} \\ 
\midrule

MB-v2  & \begin{tabular}[c]{@{}l@{}}AMC\\ Meta-Pruning\\NetAdapt\\ \textbf{GNN-RL}\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}27\%\\ 27\%\\25\%\\ \textbf{42\%}\\ \end{tabular}           & \begin{tabular}[c]{@{}l@{}}70.80\\ 71.20\\ 70.00\\70.04\end{tabular}                 & \begin{tabular}[c]{@{}l@{}}-1.00\\ -3.50\\  N/A\\ -1.83\end{tabular}        \\
\bottomrule
\end{tabular}%
% }
% \end{table}
